Deep Implicit Moving Least-Squares Functions for 3D Reconstruction

Point set is a flexible and lightweight representation widely used for 3D deep learning. However, their discrete nature prevents them from representing continuous and fine geometry, posing a major issue for learning-based shape generation. In this work, we turn the discrete point sets into smooth surfaces by introducing the well-known implicit moving least-squares (IMLS) surface formulation, which naturally defines locally implicit functions on point sets. We incorporate IMLS surface generation into deep neural networks for inheriting both the flexibility of point sets and the high quality of implicit surfaces. Our IMLSNet predicts an octree structure as a scaffold for generating MLS points where needed and characterizes shape geometry with learned local priors. Furthermore, our implicit function evaluation is independent of the neural network once the MLS points are predicted, thus enabling fast runtime evaluation. Our experiments on 3D object reconstruction demonstrate that IMLSNets outperform state-of-the-art learning-based methods in terms of reconstruction quality and computational efficiency. Extensive ablation tests also validate our network design and loss functions.

==> tables/image-table.tex <==
\begin{table}[t]
  \centering
  \scalebox{0.8}{
  \begin{tabular}{cccc}
  \toprule
 \textbf{ Network }            & \textbf{CD-$L_1$  $\downarrow$  }       &   \textbf{NC  $\uparrow$}    & \textbf{IoU $\uparrow$} \\
  \midrule
  3D-R2N2 & 0.278 & 0.695 & 0.493\\
  PointGen &  0.215 & -  & -\\
  Pix2Mesh & 0.216 & 0.772 & 0.480\\
  %IM-Net & ?? & ?? & ?? \\
  AtlasNet &  0.175  &  0.811 & - \\
  %Adaptive O-CNN  &  ? &  ? &  ?  \\
  O-Net  &  0.215 &  0.834 &  0.571   \\
  IMLS-Net  &  ? &  ? &  ?  \\
  \bottomrule
  \end{tabular}
  }
  \caption{Quantitative evaluation of different networks on the task of 3D object reconstruction from a single image. Some statistics are taken from the paper~\protect\cite{Mescheder2019}.
  }
  \label{tab:image}
  \vspace{-2mm}
  \end{table}

